Certifying Robustness of Learning-Based Keypoint Detection and Pose Estimation Methods

This work addresses the certification of the local robustness of vision-based two-stage 6D object pose estimation. The two-stage method for object pose estimation achieves superior accuracy by first employing deep neural network-driven keypoint regression and then applying a Perspective-n-Point (PnP) technique. Despite advancements, the certification of these methods' robustness remains scarce. This research aims to fill this gap with a focus on their local robustness on the system level--the capacity to maintain robust estimations amidst semantic input perturbations. The core idea is to transform the certification of local robustness into neural network verification for classification tasks. The challenge is to develop model, input, and output specifications that align with off-the-shelf verification tools. To facilitate verification, we modify the keypoint detection model by substituting nonlinear operations with those more amenable to the verification processes. Instead of injecting random noise into images, as is common, we employ a convex hull representation of images as input specifications to more accurately depict semantic perturbations. Furthermore, by conducting a sensitivity analysis, we propagate the robustness criteria from pose to keypoint accuracy, and then formulating an optimal error threshold allocation problem that allows for the setting of a maximally permissible keypoint deviation thresholds. Viewing each pixel as an individual class, these thresholds result in linear, classification-akin output specifications. Under certain conditions, we demonstrate that the main components of our certification framework are both sound and complete, and validate its effects through extensive evaluations on realistic perturbations. To our knowledge, this is the first study to certify the robustness of large-scale, keypoint-based pose estimation given images in real-world scenarios.

==> verification.tex <==
\section{Verification of ResNet}
\begin{figure}[tb]
    \centering
    \includegraphics[width=\linewidth]{img/overview.png}
    \caption{The user provides the network, the safety property to check, and desired solvers. ModelVerification.jl provides an assertion whether the safety property holds.}
    \label{fig:overview}
\end{figure}


\begin{table}[tb]
    \centering
    \begin{tabularx}{\linewidth}{@{}>{\hsize=.5\hsize}X>{\hsize=1.25\hsize}X>{\hsize=1.25\hsize}X@{}}
        \toprule
        & \textbf{NeuralVerification.jl} & \textbf{ModelVerification.jl} \\ 
        \midrule
        Supported layers & 
        Linear, ReLU, Identity & 
        Linear, ReLU, Identity, Convolution, Pooling, BatchNorm, Skip connection, Parallel layer\\ 
        \midrule
        Computation graph & 
        Sequential & 
        General Computation Graph (such as ResNet) \\ 
        \midrule
        Support GPU & 
        CPU only & 
        Both CPU and GPU \\ 
        \midrule
        Better time complexity & 
        Naive branch and bound, Loose over-approximation & 
        Novel and efficient branch and bound, Tight over-approximation \\ 
        \midrule
        Supported solvers & 
        Up to 2020 SOTA (Neurify, Reluplex, etc) & 
        Up to 2023 SOTA (alpha-beta Crown, ImageStar, etc) \\ 
        \midrule
        Specifications & 
        Polytope and Polytope Complement & 
        Polytope and Polytope Complement, Image convex hull. \\ 
        \bottomrule
    \end{tabularx}
    \caption{Improvement over NeuralVerification.jl}
    \label{tab:improvement}
\end{table}


Deep Neural Networks (DNN) are crucial in approximating nonlinear functions across diverse applications, such as computer vision and control. Verifying specific input-output properties can be a highly challenging task. To this end, we present ModelVerification.jl (MV) the only cutting-edge toolbox that contains a suite of state-of-the-art methods for verifying DNNs. This toolbox significantly extends and improves the previous version (NeuralVerification.jl) and is designed to empower developers and machine learning practitioners with robust tools for verifying and ensuring the trustworthiness of their DNN models. \Cref{fig:overview} shows the overview of the toolbox. The improvement over NeuralVerification.jl is summarized in \cref{tab:improvement}. We want to highlight the following features of our toolbox:
% Our toolbox supports general computational graphs, diverse type of input perturbation, and covers a wide range of state-of-the-art verifiers. :

\paragraph{General computational graph} This toolbox is designed to handle general computational graph with versatile operators, such as ResNet. The toolbox can easily extends to unseen operators and novel neural network architectures.

\paragraph{Versatile perturbation} Existing neural network verification toolbox usually focus on $L_\infty$ ball input perturbations. But we provide a wide range of perturbation types, including $L_\infty$ ball, polytope set, and image convex hull. Image convex hull is perticularly useful for semantic perturbations, which has not appeared in any previous toolbox.

\paragraph{Rich collection of verifiers} There are a lot of existing verifiers. They have different advantages and disadvantages, and therefore have different best use scenarios. However, existing toolbox usually focus on one or few of them. In contrast, our toolbox covers a wide range of state-of-the-art verifiers, including alpha-beta-crown, image-star, zonotope, etc. It enables us to pick the most appropriate solver for the given problem.

\paragraph{Flexibility} Existing state of the art verification algorithms share a similar design logic: branch and bound. Based on this, we abstract a general pipeline and modularize branching algorithms and bound algorithms. By this modular design, we make it possible to pick and combine algorithms from different literature to maximize the performance for a given problem.  

\paragraph{GPU and CPU support} Some verifiers work best on GPU while others heavily rely on CPU. We support both CPU based methods and GPU based methods. The dual support enables us to choose the verifier based on the hardware conditions.

\paragraph{Readability} The code is well structured and will be well documented. We will provide a detailed documentation and tutorials on how to use the toolbox. Users can easily add/modify solvers, support new operators, or add new type of perturbations.


\subsection{Workflow}

In general, verification algorithms follow the paradigm of \textit{Branch and Bound}, which divide the hard-to-verify problem into easier problems and conquer. This process can be summarized into three step: 1. split the input set (perturbations) into smaller set, which we call branches 2. propagate the bound through the model for a given branch. 3. check whether the bound of the final layer satisfy the output specification. Repeat or terminate the process based on the result.

The detailed workflow of MV is shown in \cref{fig:flow}. All the user has to do is to call \texttt{verify} by providing the problem and the solver. The problem includes the model to verify, input perturbation (in-spec), and desired output behavior (out-spec). The solver includes desired branch split method, branch search method, and bound propagation method. Then \texttt{verify} will call \texttt{prepare\_problem} to do some preprocessing, including convert the model to a bound computational graph, make input specification compatible with the solver, and initialize the branch bank. Then \texttt{search\_branches} will start spin untill the branch bank is empty or time out. At each iteration, a batch of unverified branches will be extracted from the branch bank.  
\texttt{prepare\_method} will convert initialize the bound of the start node of the computational graph based on these branches. \texttt{propagate} will propagte the bound from the start node to the end node of the computational graph. Then \texttt{check\_inclusion} decides whether the bound of the end node satisfies the output specification. If not, that mean we found a counterexample and the verification process can terminate. If it is, then this branch is verified and we can drop it. But more often, an unknown result will be returned. That means, the over-approximation introduced in the verification process prevent us to get a firm decision. Further refinement of the problem is required to get a concrete answer. In this case, \texttt{split\_branch} will divide this branch into smaller pieces and put them back to the branch bank for future verification.



\begin{figure}[tb]
    \centering
    \includegraphics[width=\linewidth]{img/MV_flow.png}
    \caption{Verification process of ModelVerification.jl}
    \label{fig:flow}
\end{figure}



\subsection{Code structure}

The code is divided in to several major components and placed in corresponding folders: 

\subsubsection{Branching}
In this folder, we provide multiple algorithms to divide the input set. For example, divide based on input dimensions cuts the set into halves along the largest dimension. And divide on ReLU nodes adds non-linear constraint to the set to break it into two branches such that a ReLU node has fixed activation status on either branch. Two major files in this folder are:
\begin{itemize}
    \item search.jl: algorithms to iterate over all branches, such as BFS, DFS.
    \item split.jl: algorithms to split an unknown branch, such as bisect, sensitivity analysis, etc.
\end{itemize}

\subsubsection{Propagate}
In this folder, the bound is propagated from the start node to the end nodes. Note that, for a forward propagation method, start nodes are the input node of the computational graph, and end nodes are the output nodes. But for a backward propagation method, start nodes are the output nodes and end nodes are the input nodes. We use BFS to iterate through the computational graph, and propagates the bound from nodes to nodes. One major file and a one major folder in this folder are:

\begin{itemize}
    \item propagate.jl: algorithms to propagate bound from input to output, including forward and backward.
    \item operators: This folder contains specific propagation algorithms for different operators. Different solver have different propagation algorithms.
\end{itemize}

\subsubsection{Solvers}
In this folder, we define different solvers. For each solver, we have to define its bound, how to initialize the bound, and how to check whether a bound satisfies the output spec. For example, some methods have a concrete bound, such as using a polytope set to represent the bound. However, some methods are using symbolic representations, such as alpha-beta-crown, which uses two symbolic linear bounds to over-approximate the network. Each solver corresponds to a file in this folder. 
\begin{itemize}
    \item solver.jl: This file defines the generic default methods for a solver.
    \item XXX.jl: solver files.
\end{itemize}

\subsubsection{Spec}
This folder contains the definition of input and output specifications, some helper functions to construct the specifications.
\begin{itemize}
    \item spec.jl: definition and helper functions for the specifications.
\end{itemize}

\subsubsection{Attack}
This folder contains adversarial attack methods that can be used to find counterexamples of a given specification. The attack can be done before or after the propagation. If a counterexample is found, then we can terminate the verification process.
\begin{itemize}
    \item pgd.jl: this file contains three popular adversarial attack method: FGSM, PGD attack, and Auto-PGD attack.
\end{itemize}

\subsection{Evaluation}

It is difficult to directly verify on Boeing's application and model because the input size and the model size are too large for existing methods. Therefore, we use an surrogate application with a smaller size ResNet and smaller size inputs to study the effectiveness and scalability of the verifiers.

We test two robust trained ResNets, ResNet2b and ResNet4b. ResNet-2B has 2 residual blocks: 5 convolutional layers + 2 linear layers.
ResNet-4B has 4 residual blocks: 9 convolutional layers + 2 linear layers.
We use images from Cifar-10 with occulsion perturbations. The image size is $32 \times 32$. The occlusion is a $6 \times 6$ black block and is randomly placed on the original image. Examples are shown in \cref{fig:examples} We form an image convex hull by the original image and the occluded image. The verifier is ImageZono. We set a maximum $150$ splits per instance. We verified on 100 images, the results are shown in \cref{tab:results}. All instances get concrete results. The ResNet4b model has more layers and is more robust, therefore it has more holds instance than ResNet2b.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{img/example.png}
    \caption{Examples of image and the perturbed image.}
    \label{fig:examples}
\end{figure}

\begin{table}[]
    \centering
    \begin{tabular}{cccc}
        \toprule
         & holds instance & violated instance & unknown instance \\
         \midrule
         ResNet2b & 54 & 46 & 0 \\
         ResNet4b & 72  & 28 & 0 \\
         \bottomrule
    \end{tabular}
    \caption{verification results. All instances have been verified. ResNet4b is more robust, therefore has more holds instances then ResNet2b.}
    \label{tab:results}
\end{table}


\begin{table}[]
    \centering
    \begin{tabular}{cccc}
        \toprule
         Model & layers & parameters & Total Time (s)\\
         \midrule
         ResNet2b & 7 conv + 2 linear + 6 ReLU & 112006 & 93.51 \\
         ResNet4b & 11 conv + 2 linear + 10 ReLU & 123734 & 1086.40 \\
         \bottomrule
    \end{tabular}
    \caption{Model size and verification time.}
    \label{tab:results}
\end{table}

\subsection{Future work}

For the future development of this toolbox, we want to cover the following topics

\paragraph{Performance Optimization} We want further optimize the performance of the implemented solvers. Including make the code more GPU friendly, optimizing the code structure to reduce redundant computation, and optimizing memory cost.

\paragraph{Compiled Executable} For python users, we want to generate a compiled library of this package such that users can directly call the package from python without setting up. For julia users, we want to reduce the compilation time required to import this package.

\paragraph{Detailed Documentation} We will provide a detailed documentation of this package to explain code structures and design logic. We will also provide tutorials on how to use this package and how to customize this package, such as adding new solvers, new operators, and new specifications.

